Everything Happens for a Reason: Discovering the Purpose of Actions in Procedural Text

Our goal is to better comprehend procedural text, e.g., a paragraph about photosynthesis, by not only predicting what happens, but why some actions need to happen before others. Our approach builds on a prior process comprehension framework for predicting actions' effects, to also identify subsequent steps that those effects enable. We present our new model (XPAD) that biases effect predictions towards those that (1) explain more of the actions in the paragraph and (2) are more plausible with respect to background knowledge. We also extend an existing benchmark dataset for procedural text comprehension, ProPara, by adding the new task of explaining actions by predicting their dependencies. We find that XPAD significantly outperforms prior systems on this task, while maintaining the performance on the original task in ProPara. The dataset is available at http://data.allenai.org/propara

==> future-work.tex <==


\subsection{Directions for Enhancing \ourmodel}
\label{discussion}

Although our model exploits the fact that paragraphs in ProPara describe events chronologically,
\ourmodel~does not require the input document to be a simple, linear ``script".  Instead, it only needs
to know the event ordering (including partial ordering), from which it can predict how the world changes 
and explain event dependencies.
%
However, this also implies that to apply \ourmodel~to more complex text, where the order of actions
is not given, an additional temporal reasoning component would be needed, such as \cite{ning2018improving,leeuwenberg2018temporal,ning2017structured}.
%
% Alternatively, 
One could design a system that predicted event order, state changes,
and dependencies all together, allowing \ourmodel's constraints to help in
temporal order prediction. This is an interesting future direction.

Architecturally, \ourmodel~performs joint inference for structure prediction by,
at test time, first predicting the likelihood of all state changes individually
(the logits output from the encoder), and then
using beam search to find the best global prediction, subject to the constraints and biases described.
When the domain or background knowledge is available, this strategy is typically more data-efficient
and thus advantageous when the training data is limited (e.g., ProPara contains only 390 training paragraphs).

An alternative strategy would be to model and predict all state changes jointly (e.g., as in Markov Random Fields),
possibly allowing biases to be discovered rather than imposed. We plan to explore this direction in the future, especially
for problems where more labeled data is  available.




